Tailoring Polarization in WSe$_2$ Quantum Emitters through Deterministic Strain Engineering

Quantum emitters in transition metal dichalcogenides (TMDs) have recently emerged as a promising platform for generating single photons for optical quantum information processing. In this work, we present an approach for deterministically controlling the polarization of fabricated quantum emitters in a tungsten diselenide (WSe$_2$) monolayer. We employ novel nanopillar geometries with long and sharp tips to induce a controlled directional strain in the monolayer, and we report on fabricated WSe$_2$ emitters producing single photons with a high degree of polarization $(99\pm 4 \%)$ and high purity ($g^{(2)}(0) = 0.030 \pm 0.025$). Our work paves the way for the deterministic integration of TMD-based quantum emitters for future photonic quantum technologies.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
